Generating Training Data with Language Models: Towards Zero-Shot Language Understanding

Pretrained language models (PLMs) have demonstrated remarkable performance in various natural language processing tasks: Unidirectional PLMs (e.g., GPT) are well known for their superior text generation capabilities; bidirectional PLMs (e.g., BERT) have been the prominent choice for natural language understanding (NLU) tasks. While both types of models have achieved promising few-shot learning performance, their potential for zero-shot learning has been underexplored. In this paper, we present a simple approach that uses both types of PLMs for fully zero-shot learning of NLU tasks without requiring any task-specific data: A unidirectional PLM generates class-conditioned texts guided by prompts, which are used as the training data for fine-tuning a bidirectional PLM. With quality training data selected based on the generation probability and regularization techniques (label smoothing and temporal ensembling) applied to the fine-tuning stage for better generalization and stability, our approach demonstrates strong performance across seven classification tasks of the GLUE benchmark (e.g., 72.3/73.8 on MNLI-m/mm and 92.8 on SST-2), significantly outperforming zero-shot prompting methods and achieving even comparable results to strong few-shot approaches using 32 training samples per class.

==> Figs/fewshot_num_data.tex <==
\begin{wrapfigure}{r}{0.62\textwidth}
\centering
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[width=\linewidth]{Figs/fewshot-MNLI-m.pdf}
\caption{MNLI-m.}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[width=\linewidth]{Figs/fewshot-MNLI-mm.pdf}
\caption{MNLI-mm.}
\end{subfigure}
\caption{Fine-tuning the classifier on the few-shot training set only vs. on both the few-shot and \method generated set. Dots and error bars are the average performance and the standard deviation over $5$ different few-shot training/validation sets, respectively.}
% \vspace{-1em}
\label{fig:fewshot_num_data}
\end{wrapfigure}


==> Figs/num_train_data.tex <==
\begin{wrapfigure}{r}{0.62\textwidth}
\centering
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[width=\linewidth]{Figs/MNLI-m.pdf}
\caption{MNLI-m.}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[width=\linewidth]{Figs/SST-2.pdf}
\caption{SST-2.}
\end{subfigure}
\caption{Results with different amount of generated training data used. Dots and error bars are the average performance and the standard deviation over $5$ seeds, respectively.}
% \vspace{-1em}
\label{fig:num_train_data}
\end{wrapfigure}


==> Tables/few_shot.tex <==
\begin{wraptable}{r}{8cm}
\caption{
Using \method for few-shot learning. The few-shot setup follows \cite{gao2021making}.
}
\centering
\small 
\resizebox{0.55\columnwidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Method} & \textbf{MNLI-(m/mm)} & \textbf{QQP} & \textbf{CoLA} \\
\midrule
Zero-Shot SuperGen & \fullres{72.3}{0.5}/\fullres{73.8}{0.5} & \fullres{66.1}{1.1} & \fullres{32.7}{5.5} \\
\midrule
Few-Shot Manual Prompt & \fullres{68.3}{2.3}/\fullres{70.5}{1.9} & \fullres{65.5}{5.3} & \fullres{9.3}{7.3} \\
\,\, + \method & \fullres{\textbf{73.1}}{0.9}/\fullres{\textbf{74.3}}{0.6} & \fullres{\textbf{69.9}}{2.5} & \fullres{\textbf{45.5}}{6.5} \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
\label{tab:few_shot}
\end{wraptable}


==> Tables/kd_res.tex <==
\begin{wraptable}{r}{6.5cm}
\caption{
Comparisons with using CTRL for zero-shot prompting and for knowledge distillation. $^\dagger$: The entire training set is used as unlabeled data. 
}
\centering
\small 
\resizebox{0.45\columnwidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Method} & \textbf{MNLI-(m/mm)} & \textbf{SST-2} \\
\midrule
SuperGen & \fullres{\textbf{72.3}}{0.5}/\fullres{\textbf{73.8}}{0.5} & \fullres{\textbf{92.8}}{0.6} \\
CTRL Prompting & \fullres{38.5}{0.0}/\fullres{39.2}{0.0} & \fullres{72.5}{0.0} \\
Knowledge Distill$^\dagger$ & \fullres{40.8}{0.5}/\fullres{41.5}{0.6} & \fullres{73.6}{0.8} \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
\label{tab:kd_res}
\end{wraptable}


==> Tables/plm-ablation.tex <==
% \begin{table}[t]
\begin{wraptable}{r}{6.5cm}
\caption{
Results with different generator/classifier PLMs.
}
% \vspace{1em}
\centering
\small 
\resizebox{0.45\columnwidth}{!}{
\begin{tabular}{l*{2}{c}}
\toprule
{\textbf{PLMs} ($G_{\theta}$/$C_{\phi}$)} & \textbf{MNLI-(m/mm)} & \textbf{SST-2} \\ 
\midrule
CTRL/COCO-LM & \fullres{\textbf{72.3}}{0.5}/\fullres{\textbf{73.8}}{0.5} &  \fullres{92.8}{0.6} \\
CTRL/RoBERTa & \fullres{69.0}{0.8}/\fullres{70.6}{0.9} &  \fullres{\textbf{93.0}}{1.5} \\
GPT-2/COCO-LM & \fullres{69.5}{1.2}/\fullres{71.3}{1.3} & \fullres{88.2}{1.8} \\
GPT-2/RoBERTa & \fullres{68.3}{0.9}/\fullres{69.7}{0.7} & \fullres{88.6}{0.8} \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
\label{tab:plm_ablation}
\end{wraptable}
% \end{table}

